Nonlinear effects in the black hole ringdown: absorption-induced mode excitation

Gravitational-wave observations of black hole ringdowns are commonly used to characterize binary merger remnants and to test general relativity. These analyses assume linear black hole perturbation theory, in particular that the ringdown can be described in terms of quasinormal modes even for times approaching the merger. Here we investigate a nonlinear effect during the ringdown, namely how a mode excited at early times can excite additional modes as it is absorbed by the black hole. This is a third-order secular effect: the change in the black-hole mass causes a shift in the mode spectrum, so that the original mode is projected onto the new ones. Using nonlinear simulations, we study the ringdown of a spherically-symmetric scalar field around an asymptotically anti-de Sitter black hole, and we find that this "absorption-induced mode excitation" (AIME) is the dominant nonlinear effect. We show that this effect takes place well within the nonadiabatic regime, so we can analytically estimate it using a sudden mass-change approximation. Adapting our estimation technique to asymptotically-flat Schwarzschild black holes, we expect AIME to play a role in the analysis and interpretation of current and future gravitational wave observations.

==> collapse_mytable.tex <==
\begin{table}
\centering
\caption{Black hole ringdown resulting from the collapse of spheroidal ($b=16$) matter.}
\label{tb:table_collapse}
\begin{tabular}{|c|c|c|c|c|c|c|}
\toprule
\hline
{} &  $t_0-t_{\rm peak}$ &  $\delta AIC $ &  $A_{0}$ &  $A_1$ &  $A_2$ &  $A_3$ \\ \hline \midrule
\midrule
$N=0$ &               23.62 &           0.00 &     0.27 &   0.00 &   0.00 &   0.00 \\ \hline \midrule
$N=1$ &               12.75 &           0.04 &     0.28 &   1.75 &   0.00 &   0.00 \\ \hline \midrule
$N=2$ &                6.92 &           0.15 &     0.28 &   2.18 &   6.61 &   0.00 \\ \hline \midrule
$N=3$ &                4.45 &           0.19 &     0.28 &   2.18 &   8.01 &  16.20 \\ \hline \midrule
\bottomrule
\end{tabular}
\end{table}

